Explaining the Power of Topological Data Analysis in Graph Machine Learning

Topological Data Analysis (TDA) has been praised by researchers for its ability to capture intricate shapes and structures within data. TDA is considered robust in handling noisy and high-dimensional datasets, and its interpretability is believed to promote an intuitive understanding of model behavior. However, claims regarding the power and usefulness of TDA have only been partially tested in application domains where TDA-based models are compared to other graph machine learning approaches, such as graph neural networks. We meticulously test claims on TDA through a comprehensive set of experiments and validate their merits. Our results affirm TDA's robustness against outliers and its interpretability, aligning with proponents' arguments. However, we find that TDA does not significantly enhance the predictive power of existing methods in our specific experiments, while incurring significant computational costs. We investigate phenomena related to graph characteristics, such as small diameters and high clustering coefficients, to mitigate the computational expenses of TDA computations. Our results offer valuable perspectives on integrating TDA into graph machine learning tasks.

==> bettiplots.tex <==
\begin{figure*}[hbt!]
\centering
\captionsetup{justification=centering}
 \begin{subfigure}{0.32\textwidth}
 \captionsetup{justification=centering}
     \includegraphics[width=\textwidth]{figs/betti_plots/BZR.pdf}
     \caption{BZR}
     \label{fig:aa}
 \end{subfigure}
 ~
 \begin{subfigure}{0.32\textwidth}
 \captionsetup{justification=centering}
     \includegraphics[width=\textwidth]{figs/betti_plots/COX2.pdf}
     \caption{COX2}
     \label{fig:ab}
 \end{subfigure}
~
 \begin{subfigure}{0.32\textwidth}
 \captionsetup{justification=centering}
     \includegraphics[width=\textwidth]{figs/betti_plots/DHFR.pdf}
     \caption{DHFR}
     \label{fig:ac}
 \end{subfigure}
~
 \begin{subfigure}{0.32\textwidth}
 \captionsetup{justification=centering}
     \includegraphics[width=\textwidth]{figs/betti_plots/ENZYMES.pdf}
     \caption{ENZYMES}
     \label{fig:ad}
 \end{subfigure}
~
 \begin{subfigure}{0.32\textwidth}
 \captionsetup{justification=centering}
     \includegraphics[width=\textwidth]{figs/betti_plots/MUTAG.pdf}
     \caption{MUTAG}
     \label{fig:ae}
 \end{subfigure}
~
 \begin{subfigure}{0.32\textwidth}
 \captionsetup{justification=centering}
     \includegraphics[width=\textwidth]{figs/betti_plots/NCI1.pdf}
     \caption{NCI1}
     \label{fig:af}
 \end{subfigure}
~
 \begin{subfigure}{0.32\textwidth}
 \captionsetup{justification=centering}
     \includegraphics[width=\textwidth]{figs/betti_plots/PROTEINS.pdf}
     \caption{PROTEINS}
     \label{fig:ag}
 \end{subfigure}
~
 \begin{subfigure}{0.32\textwidth}
 \captionsetup{justification=centering}
     \includegraphics[width=\textwidth]{figs/betti_plots/REDDIT-MULTI-5K.pdf}
     \caption{REDDIT-MULTI-5K}
     \label{fig:ah}
 \end{subfigure}
~
 \begin{subfigure}{0.32\textwidth}
 \captionsetup{justification=centering}
     \includegraphics[width=\textwidth]{figs/betti_plots/REDDIT-MULTI-12K.pdf}
     \caption{REDDIT-MULTI-12K}
     \label{fig:ai}
 \end{subfigure}
\caption{Normalized Betti functions for features of dimensions 0, 1, and 2 across all datasets. Each Betti function has been scaled by its maximum value within the respective dataset.}
\label{fig:bettidistribution}
\end{figure*}


==> tables/robustnesstable.tex <==
\begin{table*}[h!]
\centering
\caption{\textbf{0- and 1- dimensional Robustness Accuracy Results for Graph Classification with Vietoris-Rips (VR) Using the Resistance Distance and Shortest-Path to Obtain Input Matrix.} }
\resizebox{18cm}{!}{
\begin{tabular}{c l c c c c c c c c c}
\toprule
Dist.&Perc.&BZR&COX2&DHFR&ENZYMES&MUTAG&NCI1&PROTEINS&RED-5K&RED-12K\\
\midrule
 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{SPD}}} &
5\% & 81.11 $\pm$ 4.51 & $78.51 \pm 3.16$&$61.32\pm 3.68$&$30.25\pm 2.92$&$89.47\pm 5.69$&$64.92\pm 1.99$&$71.39 \pm 1.88$&$50.54 \pm 1.28$ &\textcolor{red}{OOR}\\

&10\% & $79.75\pm 3.91$&$75.43\pm 3.77$&$60.00\pm 3.29$&$29.25\pm 2.95$&$82.37\pm 7.55$&$63.27\pm 0.84$&$71.75\pm 3.44$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\

&15\% &$78.64\pm 4.73$&$78.40\pm 4.99$&$58.09\pm 3.15$&$28.17\pm 3.14$&$84.47\pm 6.01$&$63.69\pm 1.68$&$71.39\pm 3.27$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\

\midrule

 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{RD}}} &
5\% & 78.64 $\pm$ 3.19& 77.98 $\pm$ 3.13&$59.93\pm 4.22$&$30.00\pm 3.12$&$81.58\pm 6.33$&$61.61\pm 1.13$&$72.38 \pm 3.47$&\textcolor{red}{OOR} &\textcolor{red}{OOR}\\

&10\% & $80.26\pm 3.77$&$78.09\pm 3.10$&$58.68\pm 3.48$&$27.83\pm 4.14$&$81.84\pm 6.62$&$63.35\pm 1.79$&$71.70\pm 2.59$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\

&15\% &$78.89\pm 2.88$&$77.77\pm 4.09$&$61.05\pm 3.04$&$27.25\pm 3.49$&$85.79\pm 5.58$&$62.94\pm 1.62$&$70.40\pm 3.22$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\
 
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[h!]
\centering
\caption{\textbf{0- dimensional Robustness Accuracy Results for Graph classification with Vietoris-Rips (VR) Using the Resistance Distance and Shortest-Path to Obtain Input Matrix.} }
\resizebox{18cm}{!}{
\begin{tabular}{c l c c c c c c c c c}
\toprule
Dist.&Perc.&BZR&COX2&DHFR&ENZYMES&MUTAG&NCI1&PROTEINS&RED-5K&RED-12K\\
\midrule
 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{SPD}}} &
5\% & 80.37 $\pm$ 5.44 & $77.23 \pm 2.36$&$59.87\pm 4.61$&$26.00\pm 4.32$&$84.47\pm 4.01$&$63.11\pm 1.80$&$73.05 \pm 3.42$&$43.26 \pm 2.04$ &\textcolor{red}{OOR}\\

&10\% & $79.88\pm 5.43$&$78.09\pm 2.89$&$59.67\pm 4.47$&$26.58\pm 2.53$&$86.58\pm 4.20$&$62.75\pm 0.89$&$72.83\pm 1.85$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\

&15\% &$80.12\pm 3.26$&$77.23\pm 4.49$&$60.92\pm 2.45$&$23.67\pm 3.22$&$83.95\pm 5.33$&$62.76\pm 1.42$&$70.85\pm 2.94$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\

\midrule

 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{RD}}} &
5\% & 78.40 $\pm$ 3.20& 78.94 $\pm$ 4.51&$59.41\pm 3.64$&$29.75\pm 4.05$&$81.05\pm 5.79$&$62.52\pm 1.38$&$71.75 \pm 2.55$&\textcolor{red}{OOR} &\textcolor{red}{OOR}\\

&10\% & $79.88\pm 4.87$&$78.19\pm 4.41$&$61.05\pm 2.50$&$26.75\pm 2.95$&$81.84\pm 4.01$&$62.12\pm 1.14$&$71.26\pm 3.31$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\

&15\% &$79.75\pm 3.96$&$77.45\pm 3.78$&$59.64\pm 3.37$&$26.25\pm 2.33$&$83.16\pm 5.44$&$62.97\pm 1.56$&$71.17\pm 1.93$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\
  

\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[h!]
\centering
\caption{\textbf{1- dimensional Robustness Accuracy Results for Graph Classification with Vietoris-Rips (VR) Using the Resistance Distance and Shortest-Path to Obtain Input Matrix.} }
\resizebox{18cm}{!}{
\begin{tabular}{c l c c c c c c c c c}
\toprule
Dist.&Perc.&BZR&COX2&DHFR&ENZYMES&MUTAG&NCI1&PROTEINS&RED-5K&RED-12K\\
\midrule
 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{SPD}}} &
5\% & 79.26 $\pm$ 2.78 & $78.09 \pm 2.25$&$60.79\pm 2.96$&$25.33\pm 2.87$&$81.32\pm 6.50$&$61.80\pm 1.38$&$68.48 \pm 2.20$&$44.51 \pm 1.24$ &\textcolor{red}{OOR}\\

&10\% & $79.75\pm 4.36$&$77.66\pm 4.76$&$58.62\pm 4.67$&$25.92\pm 5.05$&$80.79\pm 4.31$&$60.61\pm 1.86$&$69.10\pm 3.65$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\

&15\% &$77.41\pm 3.35$&$77.45\pm 4.65$&$61.38\pm 3.16$&$26.50\pm 2.03$&$76.05\pm 5.61$&$59.50\pm 1.80$&$67.44\pm 2.11$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\

\midrule

 \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{RD}}} &
5\% & 76.79 $\pm$ 3.63& 79.04 $\pm$ 3.40&$59.54\pm 3.80$&$22.75\pm 5.44$&$83.68\pm 6.66$&$61.66\pm 1.25$&$60.94 \pm 2.34$&\textcolor{red}{OOR} &\textcolor{red}{OOR}\\

&10\% & $78.64\pm 3.59$&$75.43\pm 2.94$&$61.38\pm 3.19$&$24.58\pm 2.58$&$76.05\pm 4.72$&$61.07\pm 1.31$&$62.56\pm 2.96$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\

&15\% &$76.91\pm 4.73$&$77.66\pm 3.09$&$58.68\pm 3.34$&$23.25\pm 4.26$&$75.79\pm 6.54$&$60.65\pm 1.81$&$65.87\pm 2.91$&\textcolor{red}{OOR}&\textcolor{red}{OOR}\\
  

\bottomrule
\end{tabular}
}
\end{table*}

==> vectorization.tex <==
\subsubsection{Vectorizations of Persistence Diagrams}

PDs are useful to shape descriptors of data \cite{hensel2021survey}. However, due to their non-vector form, we cannot use them directly as inputs in our machine-learning pipeline. A common remedy to address this issue is to construct a summary function from a given PD and vectorize it using a sequence of scale values. We use a vectorized Betti function which is one of the simplest functional summaries of PDs\cite{edelsbrunner2022computational}. Similarly, we employ two other vectorization methods, \textit{\textemdash persistent landscapes, persistent silhouette and kernels \textemdash}\cite{otter2017roadmap,hensel2021survey} to summarize the information in a PD. The mentioned summary functions are defined below.

%% new addition
\begin{definition}\label{Betti}
	Let $D=\{(b_i,d_i)\}_{i=1}^n$ be a persistence diagram (of homological dimension $p$). The Betti function (associated with $D$ and $p$) is defined as 
	\begin{equation}\label{eqn:betti_function}
	\beta_p(t)=\sum_{i=1}^nw(b_i,d_i)\chi_{[b_i,d_i)}(t),    
	\end{equation}
	where $w:\{(x,y)\in\mathbb{R}^2:x\leq y\}\rightarrow \mathbb{R}$ is a weight function and $\chi_{[b,d)}(t)=1$ if $t\in[b,d)$ and 0 otherwise. 
\end{definition}

The weight function $w$ is typically a non-decreasing function of $d-b$ (persistence). We use $w\equiv 1$ in our experiments. In this case, $\beta_p(t)$ is called the $p$-th Betti number which represents the number of $p$-dimensional holes (connected components if $p=0$, loops if $p=1$, voids if $p=2$ etc.) in the simplicial complex (corresponding to scale value $t$) within a filtration which are "born" at or before $t$ and still persistent. 

\begin{definition}[\textbf{Persistence Landscape (PL)}]\cite{bubenik2015statistical}\label{PL}
The $k$-th order landscape function of a persistence diagram $D=\{(b_i,d_i)\}_{i=1}^n$ (of homological dimension $p$) is defined as 
$$
\lambda_p(k,t) \coloneqq \hbox{kmax}_{1\leq i\leq n}f_{(b_i,d_i)}(t),
$$ 
where $f_{(b,d)}(t) = \max\{0,\min\{t-b,d-t\}\}$ and $\hbox{kmax}$ denotes the $k$-th largest element of the set. 
\end{definition}  

Persistence Silhouette (PS) is a variation of a PL which takes the form of a weighted average of the tent functions $f_{(b,d)}(t)$ as in Definition \ref{PL}.
\begin{definition}[\textbf{Persistence Silhouette (PS)}]\cite{chazal2014stochastic}  The $k$-th power silhouette function of a persistence diagram  $D=\{(b_i,d_i)\}_{i=1}^n$ (of homological dimension $p$) is defined by
$$
\phi_p^{(k)}(t) = \dfrac{\sum_{i=1}^n |d_i - b_i|^k f_{(b_i,d_i)}(t)}{\sum_{i=1}^n |d_i - b_i|^k}.
$$
\end{definition}

A summary function is vectorized by evaluating it at each point of an increasing sequence of scale values $\{t_1,t_2,…,t_d\}$ to produce a vector in $\mathbb{R}^d$.

The space of PDs can be turned into a metric via the Wasserstein distance. The Wasserstein metric is very helpful for comparing underlying shape structures of data observations (such as point clouds, images, graphs, etc.) and using PDs directly in distance-based machine learning settings. However, since computing this distance involves finding an optimal matching function between a pair of PDs, its run-time cost gets high when PDs are large in size. 

\begin{definition}\label{W-distance}
The $q$-Wasserstein distance \cite{kerber2017geometry}, $q\geq 1$, between two persistence diagrams $D$ and $\tilde D$ is defined as
\begin{equation*}
	\label{w-distance}
	W_{q}(D,\tilde D)=\Big(\inf_{\gamma:D\rightarrow \tilde D} \sum_{u\in D} \|u-\gamma(u)\|_{\infty}^q \Big)^{1/q},  
\end{equation*}
where $\|\cdot\|_\infty$ is the $L_\infty$ norm on $\mathbb{R}^2$ and $\gamma$ is a bijection between $D$ and $\tilde{D}$ where the diagrams additionally contain points of the diagonal  $\Delta=\{(b,d)\in \mathbb{R}^2\ |\  b=d\}$ with infinite multiplicity. 
\end{definition}

The bijection $\gamma$ in Definition \ref{W-distance} matches an off-diagonal point in the first diagram either with its orthogonal projection onto $\Delta$ or another off-diagonal point in the second diagram. If $q=\infty$, one obtains the \emph{bottleneck} distance (with the summation being replaced by the supremum). In applications we deal with PDs consisting of finitely many points, in which case the optimal bijection realizing the infimum always exists. Note that adding additional points from $\Delta$ to a PD does not change the value of the associated Betti function $\beta_p(t)$ since $\chi_{[a,b)}(t)=0$ whenever $a=b$. 

Under certain conditions, PDs are known to be stable [citation] with respect to perturbations in data. Naturally, it is desirable to have similar stability properties for the vector summary one is working with. Below we prove a stability result for the Betti function when the weight $w$ in Definition \ref{Betti} is the identity function. To ease the notation we drop the reference to the homological dimension of a PD and the associated Betti function. 

\begin{lemma}\label{lemma:stability}
	Then for any $u=(a,b)$ and $v=(c,d)$ with $a\leq b$ and $c\leq d$, we have
	\begin{equation*}
		\int_{\mathbb{R}}|\chi_{[a,b)}(t)-\chi_{[c,d)}(t)|dt \leq  2\|u-v\|_\infty,
	\end{equation*}
\end{lemma}
\begin{proof}
	The lemma will be proven by considering three separate exhaustive cases. Let $g(t)=|\chi_{[a,b)}(t)-\chi_{[c,d)}(t)|$.
	
	Case 1: $[a,b)\cap [c,d)\neq \emptyset$, $[a,b)\not\subseteq [c,d)$ and $[c,d)\not\subseteq [a,b)$. Assume, without the loss of generality, $a\leq c\leq b \leq d $. Then
	\begin{align*}
		\int_{\mathbb{R}}g(t)dt &= \int_a^c g(t)dt+\int_c^b g(t)dt+\int_b^d g(t)dt\\
		&=|c-a|+0+|d-b|\leq 2\|u-v\|_\infty.
	\end{align*}
	
	Case 2: $[a,b)\cap [c,d)= \emptyset$. Assume $a\leq b\leq c \leq d $. Then
	\begin{align*}
		\int_{\mathbb{R}}g(t)dt & = \int_a^b g(t)dt+\int_c^d g(t)dt\\
		&=|b-a|+|d-c|\\
		&\leq |c-a|+|d-b|\leq 2\|u-v\|_\infty.
	\end{align*}
	
	Case 3: $[a,b)\subseteq [c,d)$ or $[c,d)\subseteq [a,b)$. Assuming $a\leq c\leq d \leq b $, we find that
	\begin{align*}
		\int_{\mathbb{R}}g(t)dt& = \int_a^c g(t)dt+\int_c^d g(t)dt+\int_d^b g(t)dt\\
		&=|c-a|+0+|b-d|\leq 2\|u-v\|_\infty.
	\end{align*}
\end{proof}

\begin{theorem}\label{thm:stabilityBetti}
	Let $D$ and $\tilde D$ be two (finite) persistence diagrams with finite death values and let $\gamma$ be the optimal bijection between them with respect to the 1-Wasserstein distance. Denote by 
	$\beta$ and $\tilde \beta$ the Betti functions associated with $D$ and $\tilde D$. Then
	\[
	\|\beta-\tilde \beta\|_{L_1}\leq 2W_1(D,\tilde D).
	\]
\end{theorem}
\begin{proof}
	
	Let $u=(b_u,d_u)$ and $\gamma(u)=(b_{\phi(u)},d_{\phi(u)})$. Then
	\begin{align*}
		\|\beta-\tilde \beta\|_{L_1}&=\int_{\mathbb{R}} \Big|\sum_{u\in D}\Big[\chi_{[b_u,d_u)}(t)-\chi_{ [b_{\gamma(u)},d_{\gamma(u)})}(t)\Big] \Big|dt\\
		&\leq \sum_{u\in D} \int_{\mathbb{R}} \Big|\chi_{[b_u,d_u)}(t)-\chi_{[b_{\gamma(u)},d_{\gamma(u)})}(t)\Big|dt\\
		&\leq \sum_{u\in D} \|u-\gamma(u)\|_\infty \quad\quad \mbox{(by Lemma \ref{lemma:stability})}
	\end{align*}
\end{proof}
 








